Optimal LP Rounding and Linear-Time Approximation Algorithms for Clustering Edge-Colored Hypergraphs

We study the approximability of an existing framework for clustering edge-colored hypergraphs, which is closely related to chromatic correlation clustering and is motivated by machine learning and data mining applications where the goal is to cluster a set of objects based on multiway interactions of different categories or types. We present improved approximation guarantees based on linear programming, and show they are tight by proving a matching integrality gap. Our results also include new approximation hardness results, a combinatorial 2-approximation whose runtime is linear in the hypergraph size, and several new connections to well-studied objectives such as vertex cover and hypergraph multiway cut.

==> content-colorec/content-colorec.tex <==
\section{Experimental Results}
\label{sec:appexp}
\begin{table*}[t!]
	\caption{Summary statistics of datasets --- number of nodes $\lvert V \rvert$, number of (hyper)edges $\lvert E \rvert$, 
		maximum hyperedge size $r$, and number of categories $k$ --- along with \obj{}
		performance for the algorithms \emph{LP-round} (LP), \emph{Majority Vote} (MV), \emph{Cat-IsoCut} (IC), 
		\emph{ChromaticBalls} (CB) and \emph{LazyChromaticBalls} (LCB). 
		Performance is listed in terms of the approximation guarantee given by the LP lower bound (lower is better)
		and in terms of the edge satisfaction, which is the fraction of edges that are \emph{not mistakes}
		(higher is better; see \cref{eq:chromec}).
		Our LP method performs the best overall and can even find exactly (or nearly) optimal solutions
		to the NP-hard objective by matching the lower bound.
		We also report the running times for rough comparison, though our implementations are not optimized for efficiency. Due to its simplicity, MV is extremely fast.
	}
	\label{tab:allexp1}
	\centering
	\scalebox{0.95}{\begin{tabular}{l     l l l l     l l l l l     l l l l l    l l l ll}
			\toprule
			&&&&& \multicolumn{5}{c}{\textbf{Approx. Guarantee}} & \multicolumn{5}{c}{\textbf{Edge Satisfaction}} & \multicolumn{5}{c}{\textbf{Runtime (in seconds)}} \\ 
			\cmidrule(lr){6-10} \cmidrule(lr){11-15}  \cmidrule(lr){16-20}
			%\!\!\!\!\!\!\!
			\emph{Dataset} & $\lvert V \rvert$ & $\lvert E \rvert$ & $r$ & $k$ & LP  & MV   & IC   & CB   & LCB  & LP   & MV   & IC   & CB   & LCB  & LP & MV& IC & CB & LCB \\
			\midrule
			Brain & 638 & 21180 & 2 & 2 &1.0 & 1.01 & 1.27 & 1.56 & 1.41 & 0.64 & 0.64 & 0.55 & 0.44 & 0.5 & 1.8 & 0.0 & 1.9 & 0.4 & 0.8\\
			MAG-10 & 80198 & 51889 & 25 & 10 &1.0 & 1.18 & 1.37 & 1.44 & 1.35 & 0.62 & 0.55 & 0.48 & 0.45 & 0.49 & 51 & 0.1 & 203 & 333 & 699\\
			Cooking & 6714 & 39774 & 65 & 20 &1.0 & 1.21 & 1.21 & 1.23 & 1.24 & 0.2 & 0.03 & 0.03 & 0.01 & 0.01 & 72 & 0.0 & 1223 & 4.6 & 6.7\\
			DAWN & 2109 & 87104 & 22 & 10 &1.0 & 1.09 & 1.0 & 1.31 & 1.15 & 0.53 & 0.48 & 0.53 & 0.38 & 0.46 & 13 & 0.0 & 190 & 0.3 & 0.4\\
			Walmart-Trips & 88837 & 65898 & 25 & 44 & 1.0 & 1.2 & 1.19 & 1.26 & 1.26 & 0.24 & 0.09 & 0.09 & 0.04 & 0.05 & 7686 & 0.2& 68801 & 493 & 1503\\
			\bottomrule
	\end{tabular}}
\end{table*} 
